All-loop geometry for four-point correlation functions

In this letter, we consider a positive geometry conjectured to encode the loop integrand of four-point stress-energy correlators in planar $\mathcal{N}=4$ super Yang-Mills. Beginning with four lines in twistor space, we characterize a positive subspace to which an $\ell$-loop geometry is attached. The loop geometry then consists of $\ell$ lines in twistor space satisfying positivity conditions among themselves and with respect to the base. Consequently, the $\textit{loop geometry}$ can be viewed as fibration over a $\textit{tree geometry}$. The fibration naturally dissects the base into chambers, in which the degree-$4 \ell$ loop form is unique and distinct for each chamber. Interestingly, up to three loops, the chambers are simply organized by the six ordering of $x^2_{1,2}x^2_{3,4}$, $x^2_{1,4}x^2_{2,3}$ and $x^2_{1,3}x^2_{2,4}$. We explicitly verify our conjecture by computing the loop-forms in terms of a basis of planar conformal integrals up to $\ell=3$, which indeed yield correct loop integrands for the four-point correlator.

==> package.tex <==
\usepackage{jheppub}
\usepackage{amsmath}
\usepackage{multicol,bbm}
\usepackage{enumerate}
\usepackage{bibentry}
%\usepackage{epstopdf}
%\usepackage{mathtools}

%\usepackage{amssymb}
%\usepackage{amsmath}
%\usepackage{amsfonts}
%\usepackage{latexsym}
%\usepackage[pdftex]{graphicx}
%\pagestyle{plain}
%\usepackage{graphicx}
%\usepackage{color}

\usepackage{amssymb}
\usepackage{bm}
\usepackage{multirow}
%\usepackage{diagbox}
\usepackage{caption}
\usepackage{tabularx}
\usepackage{enumitem}
%\usepackage{tcolorbox}   %加入box
\usepackage{extarrows}
\usepackage{tikz}
\usepackage{verbatim} % 多行注释
\usepackage{float} % 圖表固定位置


%\graphicspath{{figures/}}  % 定义所有的 .eps 文件在 figures 子目录下

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\ba{\begin{eqnarray}}
\def\ea{\end{eqnarray}}
\def\nl{\nonumber\\}
\def\aa{a}
\def\a{\alpha}
\def\b{\beta}
\def\c{{\cdot}}
\def\d{\delta}
\def\ad{{\dot\alpha}}
\def\bd{{\dot\beta}}
\def\cd{{\dot\gamma}}
\def\dd{{\dot\delta}}
\def\thetab{\tilde\theta}
\def\Res{\mbox{Res}}
\def\ZZ{\mathcal{Z}}
\def\WW{\mathcal{W}}
\def\MM{\mathcal{M}}
\def\Eq#1{Eq.~(\ref{#1})}
\def\Li{\textrm{Li}}
\def\l{\langle}
\def\r{\rangle}
\def\SS{\mathcal{S}}
\def\MHV{\textrm{MHV}}
\def\II{\mathcal{I}}
\def\OO{\mathcal{O}}
\def\b#1{\overline{#1}}
\def\nr#1{(\ref{#1})}
\def\II{\mathcal{I}}
\def\reg{\textrm{reg.}}
\def\Fig#1{Fig.~\ref{#1}}
\def\ibar{\bar{i}}
\def\jbar{\bar{j}}
\def\kbar{\bar{k}}
\def\sub#1{\textrm{#1}}
\def\CP1{\mathbb{CP}^1}
\def\SL2C{\mathrm{SL}(2,\mathbb{C})}
\def\GLoneC{\mathrm{GL}(1,\mathbb{C})}
\def\GLtwoC{\mathrm{GL}(2,\mathbb{C})}
\def\Z2{\mathbb{Z}_2}
\def \bangle{ \atopwithdelims \langle \rangle}


\def\su2{{SU(2)}}




\def\eps{{\epsilon}}
\def\o{{\omega}}
\def\a{{\alpha}}
\def\si{{\sigma}}
\def\[{\left[}
\def\]{\right]}
\def\Tr{\text{Tr\,}}


\def\L{\Lambda}
\def\l{\lambda}
\def\lb{\tilde\lambda}
\def\e{\epsilon}
\def\om{\omega}
\def\s{\sigma}
\def\a{\alpha}
\def\b{\beta}
\def\th{\theta}

\def\({\left(}
\def\){\right)}
\def\[{\left[}
\def\]{\right]}
\def\lan{\langle}
\def\ran{\rangle}
\def\<{\langle}
\def\>{\rangle}
\def\Det{\rm Det~}

\def\sG{\,\slash\!\!\!\! G}
\def\sH{\slash\!\!\!\! H}
\def\pint{-\hskip-0.41cm \int}
\def\i2{\frac{i}{2}}
\def\tv{{\tilde v}}
\def\tu{{\tilde u}}
\def\tQ{{\tilde Q}}
\def\bg{{\bar g}}
\def\bphi{{\bar \phi}}
\def\bPhi{{\bar \Phi}}
\def\tQ{{\tilde Q}}
\def\bQ{{\bar Q}}
\def\bR{{\bar R}}
\def\tR{{\tilde R}}
\def\bPhi{{\bar \Phi}}
\def\tPhi{{\tilde \Phi}}
\def\hPhi{{\hat \Phi}}
\def\bq{{\bar q}}

\def\cF{{\cal F}}
\def\cC{{\cal C}}
\def\cR{{\cal R}}
\def\cO{{\cal O}}
\def\cK{{\cal K}}
\def\cN{{\cal N}}
\def\cS{{\cal S}}
\def\cH{{\cal H}}
\def\cP{{\cal P}}
\def\cY{{\cal Y}}
\def\cS{{\mathbf S}}
\def\2F1{\,_2{\rm F}_1}
\def\sumint{\sum\hspace{-1.4em}\int}

\def\blue{\color{blue}}
\def\black{\color{black}}
\newcommand{\Blue}[1]{{\color{blue}#1\color{black}}}
\newcommand{\Red}[1]{{\color{red}#1\color{black}}}


%\newcommand{\rrangle}{\rangle \hspace{-.15em} \rangle}
%\newcommand{\llangle}{\langle\hspace{-.15em}\langle}


\def\pn{\Psi}
\def\ds{\displaystyle}

\newcommand{\ft}[2]{{\textstyle\frac{#1}{#2}}}


 \def\nref#1{{(\ref{#1})}}


\newcommand{\gr}{\frac{\kappa}{2}}
\newcommand{\tr}{\operatorname{Tr}}

\newcommand{\measure}[1]{d\mu_{#1}}

%added
\usepackage{amsthm}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}

